Faults in Linux 2.6

In August 2011, Linux entered its third decade. Ten years before, Chou et al. published a study of faults found by applying a static analyzer to Linux versions 1.0 through 2.4.1. A major result of their work was that the drivers directory contained up to 7 times more of certain kinds of faults than other directories. This result inspired numerous efforts on improving the reliability of driver code. Today, Linux is used in a wider range of environments, provides a wider range of services, and has adopted a new development and release model. What has been the impact of these changes on code quality? To answer this question, we have transported Chou et al.'s experiments to all versions of Linux 2.6; released between 2003 and 2011. We find that Linux has more than doubled in size during this period, but the number of faults per line of code has been decreasing. Moreover, the fault rate of drivers is now below that of other directories, such as arch. These results can guide further development and research efforts for the decade to come. To allow updating these results as Linux evolves, we define our experimental protocol and make our checkers available.

==> resume.tex <==
En 2001, Chou \emph{et al.}\ ont publi\'e une \'etude sur les fautes
trouv\'ees par analyse statique dans les versions 1.0 \`a 2.4.1 de
Linux. Un r\'esultat majeur de cette \'etude est que le r\'epertoire
{\tt drivers} contenait jusqu'\`a 7 fois plus de fautes que d'autres
r\'epertoires.  Ce r\'esultat a inspir\'e de nombreux travaux de recherche
afin d'am\'eliorer la fiabilit\'e du code des pilotes. Toutefois, Linux
est utilis\'e \`a l'heure actuelle dans des environnements plus vari\'es, il
fourni plus de services, et un nouveau mod\`ele de d\'eveloppement a \'et\'e
adopt\'e. Quel sont l'impact de ces changements sur la qualit\'e du code?
Les pilotes sont ils toujours un probl\`eme majeur?

Afin de r\'epondre \`a ces questions, nous avons entrepris de transposer
les exp\'eriences de Chou
\emph{et al.}\ aux versions de Linux 2.6.0 \`a 2.6.33, parues entre fin
2003 et d\'ebut 2010. Nous observons que m\^eme si la taille de Linux \`a
plus que doubl\'ee durant cette p\'eriode, le nombre de fautes par ligne
de code a diminu\'e. M\^eme si les {\tt pilotes} repr\'esentent
toujours une part importante du code du noyau et contiennent le plus
de fautes, leur taux de fautes est maintenant inf\'erieur \`a celui
d'autres r\'epertoires, comme {\tt arch} (couche d'abstraction
mat\'erielle) et {\tt fs} (syst\`emes de fichiers).  De telles
informations peuvent guider de nouveau travaux de recherche et
d\'eveloppement. Afin de permettre une mise \`a jour de ces 
ces r\'esultats par des tiers au fur et \`a  mesure de l'\'evolution de Linux,
nous d\'efinissons notre protocole d'exp\'erimentation et rendons nos
outils de v\'erifications ainsi que nos r\'esultats disponibles dans une
archive publique.

